An algorithm with nearly optimal pseudo-regret for both stochastic and adversarial bandits

We present an algorithm that achieves almost optimal pseudo-regret bounds against adversarial and stochastic bandits. Against adversarial bandits the pseudo-regret is $O(K\sqrt{n \log n})$ and against stochastic bandits the pseudo-regret is $O(\sum_i (\log n)/\Delta_i)$. We also show that no algorithm with $O(\log n)$ pseudo-regret against stochastic bandits can achieve $\tilde{O}(\sqrt{n})$ expected regret against adaptive adversarial bandits. This complements previous results of Bubeck and Slivkins (2012) that show $\tilde{O}(\sqrt{n})$ expected adversarial regret with $O((\log n)^2)$ stochastic pseudo-regret.

==> sapo-notations.tex <==
\section{Summary of notations and definitions}

\begin{align*}
	T_i(s_1,s_2) &= \#\{t:s_1 \leq t \leq s_2: I_t=i\} 
	              &\text{number of plays of arm $i$} \\
	T_i(s) &= T_i(1,s) \\
	G_i(s_1,s_2) &= \sum_{t=s_1+1}^{s_2-1} x_i(t) \\
	G_i(s) &= G_i(0,s) \\
	\hG_i(s_1,s_2) &= \sum_{t=s_1+1}^{s_2-1} x_i(t) \II{I_t=i}   & \text{rewards received from arm $i$}\\
	\hG_i(s) &= \hG_i(0,s)\\
	\hmu_i(s) &= \hG_i(s)/T_i(s)  & \text{estimated mean}\\
	\width_i(s) &=  \sqrt{\Cvii\frac{\log (n/\delta)}{T_i(s)}}   & \text{confidence bounds}\\
	\lcb_i(s) &= \max\{\lcb_i(s-1),\hmu_i(s) - \width_i(s)\},\\
	\ucb_i(s) &= \min\{\ucb_i(s-1),\hmu_i(s) + \width_i(s)\}, \\  
	\lcb^*(t) &= \max_{1 \leq i \leq K} \lcb_i(t), \\  
	n^A(s) &= \min\{t: \cA(t) = \cA(s)\},  & \text{time step after the last eviction from $\cA$}\\
	\hmu_i^A(s) &= \left. \sum_{t=n^A(s)}^{s} x_i(t) \II{I_t=i} \right/  T_i^A(s),
	   & \text{estimates from the last eviction}\\
	T_i^A(s) &= \#\{t:n^A(s) \leq t \leq s: I_t=i\}, \\
	\width_i^A(s) &= \sqrt{ \Cvii\frac{\log (n/\delta)}{T_i^A(s)}} ,\\
	\lcb_i^A(s) &= \max\{\lcb_i^A(s-1),\hmu_i^A(s) - \width_i^A(s)\} ,\\ 
	\ucb_i^A(s) &= \min\{\ucb_i^A(s-1),\hmu_i^A(s) + \width_i^A(s)\}, \\
	\ucb^*(t) &= \max_i \ucb_i(t), \\  
	D_i(s_1,s_2) &= \sum_{t=s_1+1}^{s_2} [x_i(t) - \emu_i] 
	              \\  
	D_i(s) &= D_i(n_i(s),s) \\
	\hD_i(s_1,s_2) &= \sum_{t=s_1}^{s_2} [x_i(t) - \emu_i] \II{I_t=i}
	     & \text{deviation from the estimated mean}\\  
	\hD_i(s) &= D_i(n_i(s),s) \\
	L^0_i & = \lceil 2\Ciii K/\egp_i^2 \rceil 
	           & \text{minimal length of testing phase}\\
	E^0 & = \lceil \ci \cdot \log(n/\delta) \rceil 
	          & \text{maximal number of detections in Step 4.a}\\
	\numPH & = \lceil \log_2 n\rceil + 2E^0
	          & \text{maximal number of testing phases for any arm}\\
	bla
\end{align*}

\begin{eqnarray*}
	\emu_i && \text{frozen estimate of the mean}\\
	\egp_i && \text{estimate for the gap}\\
	\tau_{i,k} && \text{start time of the $k$-th testing phase for bad arm $i$}\\
	p_{ik} && \text{probability of choosing bad arm $i$ in its $k$-th testing phase}\\
	L_{ik} && \text{length parameter of the $k$-th testing phase for bad arm $i$}\\
	L_i(t) && \text{length parameter of bad arm $i$ in the testing phase containing time $t$}\\
	\nbi && \text{time when arm $i$ is evicted from $\cA$}\\
	\ns && \text{time when \sapo\ switches to \expp}\\
	bla
\end{eqnarray*}
